SPARK: Real-Time Monitoring of Multi-Faceted Programming Exercises

Monitoring in-class programming exercises can help instructors identify struggling students and common challenges. However, understanding students' progress can be prohibitively difficult, particularly for multi-faceted problems that include multiple steps with complex interdependencies, have no predictable completion order, or involve evaluation criteria that are difficult to summarize across many students (e.g., exercises building interactive web-based user interfaces). We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges. SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated tests for these checkpoints, and generates visualizations to track progress across steps. SPARK also allows instructors to inspect intermediate outputs, providing deeper insights into solution variations. We also construct a dataset of 40-minute keystroke coding data from N=22 learners solving two web programming exercises and provide empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 programming instructors.

==> sections/00_abstract.tex <==
\begin{abstract}
% Sharing students' coding progress in real-time during in-class exercises enables instructors to more effectively monitor the introductory programming classrooms. 

% This immediate insight allows instructors to quick identify students who may be struggling, or common misconceptions and challenges encountered by multiple students.
% However, in more advanced programming courses, such as UI programming, the nonlinear and component-based nature of the work presents significant challenges for tracking and comparing students' progress. 
% The complexity and independence of UI components can result in varied development paths, making it difficult for instructors to maintain a consistent overview of the students' progress.
% To address this challenge, 

% In large-scale User Interface (UI) programming classes, real-time UI programming exercises are important for  learning. 
% However, the nonlinear and component-based nature of UI tasks makes tracking students' progress on UI components challenging. 


% VERSION 1:
% Monitoring in-class programming exercises offers real-time insights, helping instructors quickly identify struggling students or common misconceptions. However, this becomes challenging when exercises involve non-linear solution paths with nested substeps, where some steps are interdependent and others independent (e.g., in web programming). We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges. SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated testing for these checkpoints, and generates visualizations to track progress. It also enables inspection of intermediate outputs at each checkpoint, providing deeper insights into solution variations. In addition to the design of SPARK, we constructed a dataset of 40 minutes keystroke coding data from N=22 learners solving two web programming exercises, collected from a custom code editor extension. We also provided empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 participants with programming teaching experience.

% VERSION 2 (APRIL):
% Monitoring in-class programming exercises offers real-time insights, helping instructors quickly identify struggling students or common misconceptions. However, this becomes challenging when exercises involve non-linear solution paths with nested substeps, where some steps are interdependent and others independent (e.g., in web programming). We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges. SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated testing for these checkpoints, and generates visualizations to track progress. It also enables inspection of intermediate outputs at each checkpoint, providing deeper insights into solution variations. In addition to the design of SPARK, we constructed a dataset of 40 minutes keystroke coding data from N=22 learners solving two web programming exercises, collected from a custom code editor extension. We also provided empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 participants with programming teaching experience.

% VERSION 3 (STEVE):
Monitoring in-class programming exercises can help instructors identify struggling students and common challenges. However, understanding students' progress can be prohibitively difficult, particularly for multi-faceted problems that include multiple steps with complex interdependencies, have no predictable completion order, or involve evaluation criteria that are difficult to summarize across many students (e.g., exercises building interactive web-based user interfaces). We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges. SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated tests for these checkpoints, and generates visualizations to track progress across steps. SPARK also allows instructors to inspect intermediate outputs, providing deeper insights into solution variations. We also construct a dataset of 40-minute keystroke coding data from N=22 learners solving two web programming exercises and provide empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 programming instructors.

% In-class programming exercises are a key learning method for students, as they provide hands-on experience with newly learned concepts and allow for immediate feedback. 
% However, in large scale web programming classes, the nonlinear code structure and multi-level requirements of web programming exercises makes it challenging for instructors to effectively monitor and assess student's progress in real-time, thereby reducing their ability to provide targeted feedback. 
% In this paper, we introduce SPARK, a system designed for real-time web programming exercises monitoring, providing instructors with multi-level insights into students' progress, performance, and challenges encountered. SPARK’s monitoring operates on three levels. 
% The first level involves using customized multi-level checkpoints visualization to gain a comprehensive understanding of  students’ progress. 
% The second level employs simulated interaction inspections to track variations in element behavior, enabling the identification and resolution of potential issues. 
% Based on these insights, instructors can identify students who need assistance and directly access their code to provide feedback. 

% A within-subjects user study demonstrated that SPARK enhances instructors' ability to understand students' programming progress and deliver more targeted feedback more efficiently. 

% 1. Help identify students who are falling behind and where they are stuck. - progress viz
% 2. Identify why they are falling behind. - progress viz and class statistics
% 3. Review the output to understand the issues they are facing.  - inspector
% 4. Access the code box to more easily diagnose problems, as the observed issues provide a preliminary understanding. - code box and code box statistics
% 5. Provide personalized feedback more effectively.

% In this paper, we introduce SPARK, a system designed for real-time monitoring of web programming exercises. SPARK leverages customized multi-level checkpoint visualization and simulated interaction inspections to track variations in element behavior to support comprehensive real-time monitoring. Customized multi-level checkpoints visualization allows instructors to gain multi-level insights about detailed students’ progress change.  Element inspections allows instructors to view attribute and visual variations directly to allowing them to identify and address potential issues more effectively.




\end{abstract}

==> sections/_scratchpad.tex <==
% April's Attempt of the Abstract

Monitoring in-class programming exercises offers real-time insights, helping instructors quickly identify struggling students or common misconceptions.
However, this becomes challenging when exercises involve non-linear solution paths with nested substeps, where some steps are interdependent and others independent (e.g., in web programming).
We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges.
SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated testing for these checkpoints, and generates visualizations to track progress.
It also enables inspection of intermediate outputs at each checkpoint, providing deeper insights into solution variations.
In addition to the design of SPARK, we constructed a dataset of 30 minutes keystroke coding data from N=20 learners solving two web programming exercises, collected from a custom code editor extension.
We also provided empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 instructors and teaching assistants.

==> table/figure1.tex <==
\begin{teaserfigure}
    \centering
    \includegraphics[width=1.0\linewidth]{sections/overview.pdf}
    \caption{\sys{} consists of five panels. Here's an overview of the \sys{} dashboard: the \textit{Reference Panel} (a), which provides instructors with the expected code answer, the webpage, and a DOM tree preview for the programming exercise; the \textit{Checkpoints Panel} (b), which allows for the creation and display of nested-task checkpoints; the \textit{Progress Visualization} (c), which presents a visualization of students' programming progress; the \textit{Component Inspector} (d), which enables instructors to customize inspections of students' output variations; and the \textit{My Classroom} (e), which contains student code and statistics on overall task performance.
    %\fixme{Make the caption more explanatory}
    }
    \label{overview}
\end{teaserfigure}

==> table/table1.tex <==
\begin{table}[htbp] 
\centering
\caption{We recruited 16 participants with teaching experience and were familiar with web programming.}
\renewcommand{\arraystretch}{1.2} % Adjusts the row height for readability
\begin{tabular}{ccccccccc}
% \hline
\textbf{PID} & \textbf{Gender} & \textbf{Web Prog. Proficiency}     \\ 
\hline
1  & Female & Intermediate   \\ 
2  & Female & Intermediate   \\ 
3  & Male & Intermediate   \\ 
4  & Female & Beginner   \\ 
5  & Female & Intermediate   \\
6  & Female & Beginner   \\ 
7  & Female & Intermediate   \\ 
8  & Female & Advanced   \\ 
9  & Female & Intermediate   \\ 
10 & Male & Beginner   \\ 
11 & Female & Beginner   \\ 
12 & Female & Beginner   \\ 
13 & Female & Intermediate   \\ 
14 & Male & Intermediate   \\ 
15 & Female & Beginner   \\ 
16 & Male & Intermediate   \\ 
17 & Male & Intermediate   \\ 
18 & Female & Beginner   \\ 
19 & Female & Intermediate   \\ 
20 & Female & Beginner   \\ 
21 & Male & Beginner   \\ 
22 & Female & Beginner   \\ 
\hline
\end{tabular}
\label{tableweb}
\end{table}


\begin{table}[htbp] 
\centering
\caption{We recruited 16 participants with teaching experience and were familiar with web programming.}
\renewcommand{\arraystretch}{1.2} % Adjusts the row height for readability
\begin{tabular}{ccccccccc}
% \hline
\textbf{PID} & \textbf{Gender} & \textbf{Web Prog. Exp.} & \textbf{Teaching Exp.}    \\ 
\hline
1  & Male & 1 year & Teaching Assistant   \\ 
2  & Female & 2 years & Teaching Assistant \\
3  & Female & 1 year & Teaching Assistant \\
4  & Female & 1 year & Teaching Assistant \\
5  & Female & 2 year & Teaching Assistant \\
7  & Female & 3 years & Teaching Assistant \\
8  & Male & 1 year & Instructor \\
9  & Male & More than 6 years &Teaching Assistant \\
10 & Male & 3 years &Tutor\\
11 & Female & 1 year &Teaching Assistant \\
12 & Female & 2 years & Tutor \\
13 & Female & 3 years & Instructor \\
14 & Female & 2 years & Teaching Assistant \\
15 & Male & 3 years & None \\
16 & Male & 2 years & Teaching Assistant \\
\hline
\end{tabular}
\label{table1}
\end{table}
